Posterior Sampling in High Dimension via Diffusion Processes

Sampling from the posterior is a key technical problem in Bayesian statistics. Rigorous guarantees are difficult to obtain for Markov Chain Monte Carlo algorithms of common use. In this paper, we study an alternative class of algorithms based on diffusion processes and variational methods. The diffusion is constructed in such a way that, at its final time, it approximates the target posterior distribution. The drift of this diffusion is given by the posterior expectation of the unknown parameter vector ${\boldsymbol \theta}$ given the data and the additional noisy observations. In order to construct an efficient sampling algorithm, we use a simple Euler discretization of the diffusion process, and leverage message passing algorithms and variational inference techniques to approximate the posterior expectation oracle. We apply this method to posterior sampling in two canonical problems in high-dimensional statistics: sparse regression and low-rank matrix estimation within the spiked model. In both cases we develop the first algorithms with accuracy guarantees in the regime of constant signal-to-noise ratios.

==> TAP.tex <==
\section{Sampling algorithms based on minimizing the TAP free energy}
\label{sec:TAP}

An alternative method that effectively estimates the posterior mean vectors involves minimizing the Thouless-Anderson-Palmer (TAP) free energy.  
This section introduces sampling algorithms developed based on this approach.
We also provide theoretical guarantees that accompany. 
The results presented here are applicable to a much broader class of prior distributions, and encompass both high-dimensional regression and low-rank matrix estimation problems.

This section is organized as follows: \yw{todo} 

\subsection{Posterior sampling from high-dimensional linear models}

We consider the following high-dimensional linear model:
%
\begin{align}
\label{eq:LR}
	\by = \bX \bbeta_0 + \bepsilon \in \RR^n. 
\end{align}
%
In the above display, $\bX \in \RR^{n \times p}$ is the design matrix, $\bbeta_0 \in \RR^p$ collects the true coefficients, and $\bepsilon \in \RR^n$ stands for the noise vector. 
We further assume $\bbeta_0$ follows a product prior: $\beta_{0, i} \iidsim \pi_{\beta}$, where $\pi_{\beta}$ is a fixed prior distribution over $\RR$ that does not change with $(n, p)$.

Given observations $(\bX, \by)$, our goal is to draw samples from the posterior distribution of the linear coefficients $\bbeta_0$. 
To this end, we shall construct the diffusion processes associated with model \eqref{eq:LR}. 
Following the previous discussions, there are at least two ways of doing it: 
%
\begin{enumerate}
	\item To sample from the posterior distribution of the linear coefficients, we may track the stochastic localization process $\dd \bz(t) = \bm(\bz(t), t) \dd t + \dd \bB(t)$ that is initialized at the origin. For the linear regression setting that we consider, $\bm(\bz(t), t) = \E[\bbeta_0 \mid \bX, \by, \bz(t)]$. Here, $\bz(t) = t \bbeta_0 + \bG(t) \in \RR^p$, and $(\bG(t))_{t \geq 0}, (\bB(t))_{t \geq 0}$ are $p$-dimensional standard Brownian motions. Approximating $\bz(T)$ for a sufficiently large $T$ then gives approximate samples from the target posterior distribution. 
	\item Alternatively, we may consider the linear observation process $\dd \by(t) = \bm_y(\by(t), t) \dd t + \dd \bB_y(t)$ that is once again initialized at the origin, where $\bm_y(\by(t), t) = \E[\bX \bbeta_0 \mid \by, \bX, \by(t) ] \in \RR^n$. We let $\by(t) = t \bX \bbeta_0 + \bG_y(t) \in \RR^n$, where  $(\bG_y(t))_{t \geq 0}, (\bB_y(t))_{t \geq 0}$ are Brownian motions in $\RR^n$. Tracking this linear observation process leads to samples from the posterior distribution of $\bX \bbeta_0$ given $(\bX, \by)$, which further requires solving a linear inverse problem to obtain linear coefficient samples. The solution is unique when $\bX$ has rank $p$. 
\end{enumerate}

Before proceeding, we state our distributional assumptions on model \eqref{eq:LR}, 
We adopt the same set of assumptions as \cite{celentano2023mean} and many other papers, which we summarize below:
%
\begin{assumption}
\label{assumption:LR}
	We assume $(\bX, \bbeta_0, \bepsilon)$ are independent of each other, with entries satisfying
	%
	\begin{align*}
		x_{ij} \iidsim \normal(0, 1 / p), \qquad \beta_{0, j} \iidsim \pi_{\beta}, \qquad \eps_i \iidsim \normal(0, \sigma^2). 
	\end{align*}
	%
	Here, $\sigma^2 > 0$ represents the noise level, $\pi_{\beta}$ is a prior distribution over $\RR$ that has a compact support with at least three distinct values. Without loss, we assume $\pi_{\beta}$ has unit second moment. As $n, p \to \infty$, we assume $n / p \to \delta \in (0, \infty)$. We also assume $(\sigma^2, \delta, \pi_{\beta})$ are fixed and are independent of $(n, p)$. 
\end{assumption}

\begin{remark}
	If $\pi_{\beta}$ has no more than two distinct values, or in general, is discrete, then the previous set of results for spike matrix model and AMP also apply in the regression setting. The proof is similar, and we skip the proof to avoid redundancy. 
\end{remark}

\subsubsection{AMP for linear regression}
\label{sec:Bayes-AMP-LR}

We next state the AMP algorithm for model \eqref{eq:LR}, which in many regimes effectively estimates the posterior expectation $\E[\bbeta_0 \mid \bX, \by, \bz(t)]$.  

Given inputs $(\bX, \by, \bz(t))$,  the AMP algorithm refers to a class of iterative algorithms that take the following form:
%
\begin{align}
\label{eq:linear-AMP}
	\left\{
	\begin{array}{l}
		\bb^{k + 1} = \bX^{\top} f_k(\ba^k, \by) - \xi_k g_k(\bb^k, \bz(t)), \\
		\ba^k = \bX \bg_k(\bb^k, \bz(t)) - \eta_k f_{k - 1}(\ba^{k - 1}, \by), 
	\end{array} \right.
\end{align}
%
where at initialization we set $\ba^{-1} = \mathbf{0}_n$. After $k$ iterations, algorithm \eqref{eq:linear-AMP} outputs $g_k(\bb^k, \bz(t)) \in \RR^p$ as an estimate of $\bbeta_0$.  
In the above iteration, we assume $f_k, g_k: \RR^2 \to \RR$ are Lipschitz continuous and apply on matrices row-wisely (note that $f_{-1}$ maps from $\RR$ to $\RR$). The scalar sequences $(\xi_k)_{k \geq 0}$ and $(\eta_k)_{k \geq 0}$ are determined by the following state evolution recursion: 
%
\begin{align*}
	& \xi_k = \delta \E[\partial_1 f_k(\bar{G}_k, \bar{G}_{\ast} + \eps )], \qquad \eta_k =  \E[\partial_1 g_k(\mu_t B + G_k, U)], \qquad \sigma_k^2 = \delta \E[f_{k - 1}(\bar{G}_{k - 1}, \bar{G}_{\ast} + \eps)^2] \\
	&  \bar\sigma_k^2 =  \E[g_t(\mu_k B + G_k, U)^2], \qquad \bar\sigma_{k, \ast} =  \E[Bg_k(\mu_k B + G_k, U)], \qquad \mu_k = \delta \E[\partial_{2} f_{k - 1}(\bar{G}_{k - 1}, \bar{G}_{\ast} + \eps) ], %\\
	%& B \sim \pi_{\beta}, \qquad \bar{G}_{\ast} \sim \normal(0,1), \\ %\qquad  \bar\sigma_0^2 = \bar\sigma_{0,0} = 0, \\
	%&  \eps \sim \normal(0, \sigma^2), \qquad G_t \sim \normal(0, \sigma_t^2), \qquad \bar{G}_t \sim \normal(0, \bar\sigma_t^2), \qquad \E[\bar{G}_t \bar{G}_{\ast}] = \bar\sigma_{t, \ast}. 
\end{align*} 
%
where $B \sim \pi_{\beta}$, $\bar{G}_{\ast} \sim \normal(0,1)$, $\eps \sim \normal(0, \sigma^2)$, $G_k \sim \normal(0, \sigma_t^2)$, $\bar{G}_k \sim \normal(0, \bar\sigma_k^2)$, and $U \sim t B + \sqrt{t}G$. Here, $B \perp G_k$, $\eps \perp (\bar{G}_{\ast}, \bar{G}_k)$, and $(\bar{G}_{\ast}, \bar{G}_k)$ are jointly Gaussian.
We also assume $G \sim \normal(0, 1)$ and is independent of anything else.  

Choosing appropriate non-linearities, we get the Bayes AMP: 
%
\begin{align*}
	& f_k(\bar{G}_k, \bar{G}_{\ast} + \eps) = \E[\eps \mid \bar{G}_k,  \bar{G}_{\ast} + \eps], \qquad g_k(\mu_k B + G_k, U) = \E[B \mid \mu_k B + G_k, U]. 
\end{align*}
%
In this case, straightforward computation gives  $\bar\sigma_k^2 = \bar\sigma_{k, \ast}$ and $\sigma^2 \mu_k = \sigma_k^2$. In addition, the state evolution quantities admit the following expressions:  
%
\begin{align*}
	& f_k(x, y) = \frac{\sigma^2(y - x)}{\sigma^2 + 1 - \bar\sigma_k^2},  \\ %\left( \frac{1}{1 - \bar\sigma_t^2} + \frac{1}{\sigma^2} \right)^{-1} \cdot  \left(\frac{x}{1 - \bar{\sigma}_t^2} + \frac{y}{\sigma^2}\right), \\
	& g_k (x, u) = \E[B \mid (\sigma^{-2}\mu_k B + t) + \sqrt{\sigma^{-2}\mu_k + t} G = \sigma^{-2}x + u], \\
	& \mu_k = \frac{\delta\sigma^2}{\sigma^2 + 1 - \bar\sigma_{k - 1}^2}, \qquad \bar\sigma_k^2 =  \E\left[ \E[B \mid (\sigma^{-2}\mu_k + t)  B + \sqrt{\sigma^{-2}\mu_k + t} G ]^2 \right], \\
	& \xi_k = -\frac{\delta\sigma^2}{\sigma^2 + 1 - \bar\sigma_k^2}, \qquad \eta_k = \sigma^{-2}\E\left[ \Var[B \mid (\sigma^{-2}\mu_k + t)  B + \sqrt{\sigma^{-2}\mu_k + t} G] \right]. 
\end{align*}
%
We define $E_{k} := 1 - \bar\sigma_{k, \ast}$.
As initialization, we get $E_{-1} = 1$.
For $k \geq 0$ we have
%
\begin{align*}
	& E_{k} = \mmse \left( {\sigma^{-2} \mu_k} + t\right) = \mmse \left( { \delta (\sigma^2 + E_{k - 1})^{-1} } + t \right), \\
	& \mmse(\gamma) := \E\left[ \left( B - \E[B \mid \gamma B + \sqrt{\gamma} G] \right)^2 \right]. 
\end{align*}
%
Below we establish a useful property regarding Bayes AMP state evolution. 
We delay the proof to Appendix \ref{sec:proof-lemma:unique-stationary} for the compactness of presentation. 
%
\begin{lemma}
\label{lemma:unique-stationary}
	We assume $\pi_{\beta}$ is supported on $[-M_{\beta}, M_{\beta}]$.
	Then the following statements are true: 
	%
	\begin{enumerate}
		%\item If in addition $\pi_{\beta}$ is supported on finitely many points, then there exists a constant $C_{\beta} \in (0, \infty)$ that depends only on $\pi_{\beta}$, such that for all $\frac{1}{\lambda (\sigma^2 + 1)} > C_{\beta}$ and all $t > 0$, the following fixed point equation has a unique solution:
		%
	\item Recall that $\delta = \lim_{n, p \to \infty} n / p$. There exists a constant $c_{\beta} \in (0, \infty)$, such that for all $\frac{\delta^{1/2}}{\sigma^3} < c_{\beta}$, the  fixed point equation below for all $t \geq 0$ has a unique positive solution.
	%
		\begin{align}
		\label{eq:fixed-point-equation}
			E = \mmse\left(\delta (\sigma^2 + E)^{-1} + t\right). 
		\end{align}
		%
	\item  There exists a constant $C_{\beta} \in (0, \infty)$, such that for all $\delta > C_{\beta}$, the fixed point equation \eqref{eq:fixed-point-equation} has a unique positive solution for all $t \geq 0$. 
	\item Assume the conditions of claim 1 or claim 2, and denote the unique solution to fixed point equation \eqref{eq:fixed-point-equation} by $E_{\ast} (\delta, \sigma)$. Then for all $k \in \NN$,
	%
	\begin{align*}
		|E_k - E_{\ast}(\delta, \sigma, t)| \leq \frac{|1 - E_{\ast}(\delta, \sigma, t)|}{2^{k + 1}}.  
	\end{align*} 
	\end{enumerate} 
\end{lemma}
%
Fixed point equation \eqref{eq:fixed-point-equation} having a unique positive solution implies that Bayes AMP consistently estimates the posterior expectation, in the sense of the following lemma. 
%
\begin{lemma}
\label{lemma:LR-AMP-consistent}
	We assume that the fixed point equation \eqref{eq:fixed-point-equation} has a unique positive solution for all $t > 0$. Then for any $\eps, T > 0$, there exists $K(T, \eps) \in \NN$ that depends only on $(\delta, \sigma^2, \pi_{\beta}, \eps, T)$, such that for any $t \leq T$, 
	%
	\begin{align*}
		\plimsup_{n, p \to \infty}  \frac{1}{\sqrt{p}} \|\bm (\bz (t), t) - g_{K(T,\eps)}(\bb^{K(T,\eps)}, \bz(t)) \|_2 \leq \eps, 
	\end{align*}
	%
	where we recall that $\bb^k$ is the $k$-th iteration of the AMP algorithm \eqref{eq:linear-AMP}.    
\end{lemma}



\subsubsection{Variational inference based on the TAP free energy}

We introduce in this section the TAP free energy. 
To set the stage, we define the following set: 
%
\begin{align*}
	\Gamma = \left\{ (m, s) \in \RR^2: \mbox{there exists }(\lambda, \gamma) \in \RR^2, \mbox{ such that }m = \langle \beta \rangle_{\lambda, \gamma} \mbox{ and }s = \langle \beta^2 \rangle_{\lambda, \gamma} \right\}, 
\end{align*}
%
where
%
\begin{align*}
	\langle f(\beta) \rangle_{\lambda, \gamma} = \int f(\beta) \pi_{\lambda, \gamma}(\diff \beta), \qquad \pi_{\lambda, \gamma}(\diff \beta) \propto e^{-\gamma \beta^2 / 2 + \lambda \beta} \pi_{\beta}(\diff \beta).
\end{align*}
%
Following the discussions in \cite{celentano2023mean}, we see that $\Gamma$ is convex and open in $\RR^2$. 
We consider the TAP free energy, defined over the domain $(\bm, \bs) \in \Gamma^p \subseteq \RR^p \times \RR^p$, 
%
\begin{align*}
	\cF_{\TAP}(\bm, \bs; t, \by, \bX, \bz(t), \sigma^2) = & \frac{n}{2} \log 2\pi \sigma^2 + D_0(\bm, \bs) + \frac{1}{2\sigma^2} \|\by - \bX\bm\|_2^2 + \frac{n}{2} \log \left( 1 + \frac{S(\bs) - Q(\bm)}{\sigma^2} \right) \\
	& + \frac{1}{2t} \|\bz(t) - t \bm\|_2^2 + \frac{tp}{2}(S(\bs) - Q(\bm)). 
\end{align*}
%
We ignore the dependency on $(\by, \bX, \bz(t), \sigma^2)$ when there is no confusion. 
In the above display, 
%
\begin{align*}
	& S(\bs) = \frac{1}{p} \sum_{j = 1}^p s_j, \qquad Q(\bm) = \frac{1}{p} \sum_{j = 1}^p m_j^2, \qquad D_0(\bm, \bs) = \sum_{j = 1}^p -h(m_j, s_j), \\
	&  -h(m, s) = \sup_{(\lambda, \gamma) \in \RR^2}  - \frac{1}{2}\gamma s + \lambda m - \log \E_{\beta \sim \pi_{\beta}}\left[ e^{-\gamma \beta^2 / 2 + \lambda \beta} \right].
\end{align*}
%
We define the posterior first and second moment vectors as 
%
\begin{align*}
	\bm_{\sB, t} = \E[\bbeta_0 \mid \bX, \by, \bz(t)], \qquad \bs_{\sB, t} = \E[\bbeta_0^2 \mid \bX, \by, \bz(t)], 
\end{align*}
%
both are in $\RR^p$. 
In the sequel, we shall prove the existence of a local minimizer of the TAP free energy $\cF_{\TAP}(\bm, \bs; t)$ over $(\bm, \bs) \in \Gamma^p$, near the true posterior first and second moments.
To this end, we establish the local convexity of TAP free energy. 

\subsubsection{Convexity of the TAP free energy}


Note that the signal-to-noise ratio (SNR) of the linear regression problem \eqref{eq:LR} is influenced by at least two factors: the limiting aspect ratio $\delta$ and the noise level $\sigma^2$. 
To elaborate, a large $\delta$ and a small $\sigma^2$ imply a high SNR, and vice versa. 

Below, we discuss two separate theorems that  correspond to sufficiently high and low SNRs. We start with the low SNR regime, and show that the TAP free energy is globally strongly convex in this regime.
 We formally state this result as \cref{lemma:low-SNR}, which  is a direct consequence of \cite[Proposition 3.3]{celentano2023mean}. The proof of the lemma is deferred to Appendix \ref{proof:lemma:low-SNR}. 

\begin{lemma}
\label{lemma:low-SNR}
	We assume Assumption \ref{assumption:LR}. Then there exist constants $\kappa$, $c_{\beta} > 0$ that depend only on $\pi_{\beta}$, such that if $\delta / \sigma^2 < c_{\beta}$, then for a sufficiently large $(n, p)$,  $\nabla^2 \cF_{\TAP} (\bm, \bs; t) \succeq \kappa I_{2p}$ for all $(\bm, \bs) \in \Gamma^p$.  
\end{lemma}

Without a high enough SNR, the TAP free energy might not be globally convex, and finding the associated global minimizer could be challenging. On the positive side, \cite{celentano2023mean} proved that in many cases, the TAP free energy at $t = 0$ is strongly convex in a local neighborhood of the posterior expectation.

To state their result, we need to introduce the necessary and sufficient condition for Bayes AMP to consistently estimate the posterior expectation. We describe this condition in Assumption \ref{assumption:AMP-LR-optimal}. 
As we shall see later, we do not directly impose Assumption \ref{assumption:AMP-LR-optimal}  to establish our main theorems. Instead, we will prove that Assumption \ref{assumption:AMP-LR-optimal} holds under mild conditions in certain SNR regimes. 
%
\begin{assumption}
	\label{assumption:AMP-LR-optimal}
	Recall that $\mmse(\gamma) = \E_{(B, Z) \sim \pi_{\beta} \times \normal(0, 1)}[(B - \E[B \mid \gamma B + \sqrt{\gamma} Z])^2]$. Define the replica-symmetric potential
	%
	\begin{align*}
		\phi(\gamma) = \frac{\sigma^2 \gamma}{2} - \frac{\delta}{2} \log \frac{\gamma}{2\pi \delta} + i(\gamma), 
	\end{align*}
	%
	where $i(\gamma)$ is the mutual information between $B$ and $\gamma B + \sqrt{\gamma} Z$ for $(B, G) \sim \pi_{\beta} \otimes \normal(0, 1)$. Let 
	%
	\begin{align*}
		\gamma_{\mathrm{stat}} := \argmin_{\gamma > 0} \phi(\gamma), \qquad \gamma_{\mathrm{alg}} := \inf \{\gamma > 0: \delta / \gamma - \sigma^2 \leq \mmse(\gamma) \}. 
	\end{align*}
	We then make the following assumptions on $(\delta, \sigma^2, \pi_{\beta})$:
	%
	\begin{enumerate}
		\item The global minimizer $\gamma_{\mathrm{stat}} = \argmin_{\gamma > 0} \phi(\gamma)$ exists and is unique, and $\phi''(\gamma_{\mathrm{stat}}) > 0$. 
		\item $\gamma_{\mathrm{stat}} = \gamma_{\mathrm{alg}}$. 
	\end{enumerate}
\end{assumption} 

\begin{remark}
	If we assume either the conditions of the first point in \cref{lemma:unique-stationary}, or the conditions of the second point in \cref{lemma:unique-stationary}, then the second point of  Assumption \ref{assumption:AMP-LR-optimal} automatically follows. 
\end{remark}
%
\begin{remark}
	Per the discussions that follow Assumption 2.2 in \cite{celentano2023mean}, the first point of Assumption \ref{assumption:AMP-LR-optimal} is a mild condition, in the sense that: (1) fixing any $\sigma^2 > 0$, the global minimizer $\gamma_{\mathrm{stat}}$ exists and is unique for Lebesgue a.e. $\delta > 0$, and (2) for every $\sigma^2 > 0$, the positive second derivative condition holds for Lebesgue-a.e. $\delta > 0$. 
\end{remark}

%
We next replicate Theorem 3.1 and 3.4 of \cite{celentano2023mean} below for readers' convenience, which states that with Assumptions \ref{assumption:LR} and \ref{assumption:AMP-LR-optimal}, $\cF_{\TAP}$ at $t = 0$ has a unique local minimizer around the posterior first and second moment vectors. This statement holds for all SNR. 
%
\begin{lemma}[Theorem 3.1 and 3.4 of \cite{celentano2023mean}]
\label{lemma:LR-local-convexity}
	We assume Assumptions \ref{assumption:LR} and \ref{assumption:AMP-LR-optimal}, then there exist $\eps, \kappa > 0$ such that with probability approaching 1 as $n, p \to \infty$, $\cF_{\TAP}(\bm, \bs; 0)$ has a unique local minimizer $(\bm_{\ast}, \bs_{\ast})$ in $\mathsf{B}((\bm_{\sB}, \bs_{\sB}), \eps \sqrt{p}) = \{(\bm, \bs) \in \Gamma^p: \|(\bm, \bs) - (\bm_{\sB}, \bs_{\sB})\|_2 < \eps \sqrt{p}\}$, and 
	%
	\begin{align*}
		\inf_{(\bm, \bs) \in \mathsf{B}((\bm_{\sB}, \bs_{\sB}), \eps \sqrt{p})} \lambda_{\min} \left( \nabla^2 \cF_{\TAP}(\bm, \bs; 0) \right) \geq \kappa. 
	\end{align*}
	%
	Furthermore, 
	%
	\begin{align*}
		\frac{1}{p} \left[ \|\bm_{\ast} - \bm_{\sB}\|_2^2 + \|\bs_{\ast} - \bs_{\sB}\|_2^2 \right] \toP 0. 
	\end{align*}
\end{lemma}

Given local convexity, \cite{celentano2023mean} then design a two-stage algorithm that finds a local minimizer of the TAP free energy and at the same time, outputs consistent estimates of the posterior expectation. The algorithm implements Bayes AMP in the first stage, and runs natural gradient descent (NGD) in the second. Apart from $(\bX, \by, \bz(t))$ and $t$, several additional inputs are required to implement this algorithm: the number of AMP steps $K_{\AMP}$, the number of NGD steps $K_{\mathsf{NGD}}$, NGD step size $\eta$, and the noise level $\sigma^2$.  
For the compactness of presentation, we denote this algorithm by $\cA(\bX, \by, \bz(t), t, K_{\AMP}, K_{\mathsf{NGD}}, \eta, \sigma^2)$. We refer to \cite{celentano2023mean} for a detailed implementation of $\cA(\bX, \by, \bz(t), t, K_{\AMP}, K_{\mathsf{NGD}}, \eta, \sigma^2)$. 
We state below the theoretical guarantee for this procedure: 
%
\begin{theorem}
\label{thm:LR-TAP}
We denote the output of $\cA(\bX, \by, \bz(t), t, K_{\AMP}, K_{\mathsf{NGD}}, \eta, \sigma^2)$ by $\hat \bm(\bz(t), t)$. 
	\begin{enumerate}
		\item We assume $\delta$ is sufficiently small such that the conditions of \cref{lemma:low-SNR} and the first point of \cref{lemma:unique-stationary} are satisfied. We also assume Assumption \ref{assumption:LR}. Then, for any $\eps, t> 0$, there exists $(K_{\AMP} = 0, K_{\mathsf{NGD}}, \eta)$, such that with probability $1 - o_n(1)$, it holds that 
		%
		\begin{align*}
			\frac{1}{\sqrt{p}} \| \hat \bm(\bz(t), t) - \bm(\bz(t), t) \|_2 \leq \eps. 
		\end{align*}
		%
		In addition, there exists a constant $C_1 > 0$, such that for any $\bz_1, \bz_2 \in \RR^p$,  
		%
		\begin{align*}
			\|\hat\bm(\bz_1, t) - \hat\bm(\bz_2, t)\|_2 \leq C_1 \|\bz_1 - \bz_2\|_2 + \eps \sqrt{p}. 
		\end{align*}
		\item We assume $\delta > C_{\beta}$, where $C_{\beta}$ is given in the second point of \cref{lemma:unique-stationary}. We also require
		Assumption \ref{assumption:LR}. Then, fixing $(\delta, \pi_{\beta})$, for almost every $\sigma^2 > 0$ the following statement is true: For any $\eps$, there exists $(K_{\AMP}, K_{\mathsf{NGD}}, \eta)$, such that with probability $1 - o_n(1)$, it holds that 
		%
		\begin{align*}
			\frac{1}{\sqrt{p}} \|\hat \bm(\mathbf{0}_p, 0) - \bm(\mathbf{0}_p, 0) \|_2 \leq \eps, 
		\end{align*}
		%
		where we recall that $\bm(\mathbf{0}_p, 0) = \E[\bbeta_0 \mid \bX, \by]$. 
		Below, we write $\hat \bm(\bz(t), t; \by) = \hat \bm(\bz(t), t)$ to emphasize the dependency on $\by$. Then there exists $r > 0$, such that for any $\by_1, \by_2 \in \mathsf{B}(\by, r \sqrt{n}) = \{ \bx \in \RR^n: \|\bx - \by\|_2 \leq \sqrt{n} r \}$, it holds that 
		%
		\begin{align*}
			 \|\hat\bm (\mathbf{0}_p, 0, \by_1) - \hat\bm (\mathbf{0}_p, 0, \by_2) \|_2 \leq C_2  \|\by_1 - \by_2\|_2 + \eps \sqrt{n}. 
		\end{align*}
		%
		for a positive constant $C_2$. 
	\end{enumerate}
\end{theorem}

We defer the proof of \cref{thm:LR-TAP} to Appendix \ref{proof:thm:LR-TAP}.



\subsubsection{Sampling algorithm based on stochastic localization} 

We are then ready to state our sampling algorithms and the associated theoretical guarantees. 
We first give the algorithm for the low SNR regimes as \cref{alg:LR-low-SNR}. 

\begin{algorithm}[ht]
\caption{Diffusion-based sampling for linear models in a low SNR regime}\label{alg:LR-low-SNR}
\textbf{Input: }Data $(\bX, \by)$, parameters $( K_{\mathsf{NGD}}, \eta, \delta, \sigma^2, L, \Delta)$;	
\begin{algorithmic}[1]
\State Set $\hat{\bz}_0 = \bfzero_p$;
\For{$\ell = 0,1,\cdots, L - 1$}
	\State Draw $\bw_{\ell + 1} \sim \normal(0,\id_p)$ independent of everything so far;
	\State Denote $\hat{\bm}(\hat{\bz}_\ell,\ell\Delta)$ the output of $\cA(\bX, \by, \hat{\bz}_\ell, \ell \Delta, 0, K_{\mathsf{NGD}}, \eta, \sigma^2)$
		\State Update $\hat{\bz}_{\ell + 1} = \hat{\bz}_\ell + \hat{\bm}( \hat{\bz}_\ell, \ell\Delta) \Delta + \sqrt{\Delta} \bw_{\ell + 1}$;	
	\EndFor
\State \Return $\bbeta_0^{\salg}  = \hat{\bm}(\hat{\bz}_L, L\Delta)$;
\end{algorithmic}
\end{algorithm} 

Sampling algorithms associated with high SNR regimes are presented as \cref{alg:LR-high-SNR}. 

\begin{algorithm}[ht]
\caption{Diffusion-based sampling for linear models in a high SNR regime}\label{alg:LR-high-SNR}
\textbf{Input: }Data $(\bX, \by)$, parameters $(K_{\AMP}, K_{\mathsf{NGD}}, \eta, \delta, \sigma^2, L, \Delta)$;	
\begin{algorithmic}[1]
\State Set $\hat{\by}_0 = \bfzero_n$;
\For{$\ell = 0,1,\cdots, L - 1$}
	\State Draw $\bw_{\ell + 1} \sim \normal(0,\id_n)$ independent of everything so far;
	\State Denote $\hat{\bm}(\mathbf{0}_n,0, \hat\by_{\ell})$ the output of $\cA(\bX, \frac{\hat\by_{\ell \delta} + \sigma^{-2} \by }{\sigma^{-2} + \ell \delta}, \mathbf{0}_p, 0, K_{\AMP}, K_{\mathsf{NGD}}, \eta, (\sigma^{-2} + \ell \delta)^{-1})$
		\State Update $\hat{\by}_{\ell + 1} = \hat{\by}_\ell + \bX \hat{\bm}(\mathbf{0}_n,0, \hat\by_{\ell}) \Delta + \sqrt{\Delta} \bw_{\ell + 1}$;	
	\EndFor
\State \Return $\bbeta_0^{\salg}  = \hat{\bm}(\mathbf{0}_n,0, \hat\by_{L})$;
\end{algorithmic}
\end{algorithm}

\begin{remark}
	In \cref{alg:LR-low-SNR,alg:LR-high-SNR}, we do not include the final truncation steps, as NGD are guaranteed to return a vector with entrywise upper bound $M_{\beta}$. 
\end{remark}

\begin{remark}
	One can evaluate the SNR by checking the aspect ratio $n / p$, as well as estimating the noise level $\sigma^2$. %\yw{what can we do here?}
\end{remark}


We then provide theoretical guarantees for \cref{alg:LR-low-SNR,alg:LR-high-SNR}. We prove \cref{thm:LR-main} in Appendix \ref{sec:proof-thm:LR-main}.  

\begin{theorem}
\label{thm:LR-main}
	 We denote by $\mu_{\bX, \by}^{\mathsf{alg}}$ the law of $\bbeta_0^{\mathsf{alg}}$, obtained using \cref{alg:LR-low-SNR} or \cref{alg:LR-high-SNR}, and denote by $\mu_{\bX, \by}$ the true posterior distribution. We also assume Assumption \ref{assumption:LR}. Then the following statements are true: 
	\begin{enumerate}
		\item We assume $\delta$ is sufficiently small such that the conditions of \cref{lemma:low-SNR} and the first point of \cref{lemma:unique-stationary} are satisfied. Then for any $\xi > 0$, there exist $(K_{\mathsf{NGD}}, \eta, L, \Delta)$ that depend only on $(\delta, \sigma^2, \pi_{\beta})$, such that if \cref{alg:LR-low-SNR} takes as input $(\bX, \by, K_{\mathsf{NGD}}, \eta, \delta, \sigma^2, L, \Delta)$, then with probability $1 - o_n(1)$ over the randomness of $(\bX, \by)$, 
		%
		\begin{align*}
			W_{2, p} (\mu_{\bX, \by}, \mu_{\bX, \by}^{\mathsf{alg}}) \leq \xi. 
		\end{align*}
		\item We assume $\delta > C_{\beta}$, where $C_{\beta}$ is given in the second point of \cref{lemma:unique-stationary}. Then for any $\xi > 0$, there exist $(K_{\AMP}, K_{\mathsf{NGD}}, \eta, L, \Delta)$ that depend only on $(\delta, \sigma^2, \pi_{\beta})$, such that if \cref{alg:LR-high-SNR} takes as input $(\bX, \by, K_{\AMP}, K_{\mathsf{NGD}}, \eta, \delta, \sigma^2, L, \Delta)$, then with probability $1 - o_n(1)$ over the randomness of $(\bX, \by)$, 
		%
		\begin{align*}
			W_{2, p}(\mu_{\bX, \by}, \mu_{\bX, \by}^{\mathsf{alg}}) \leq \xi. 
		\end{align*}
	\end{enumerate}
\end{theorem} 

\subsection{Posterior sampling from spiked models with continuous prior}

We revisit model \eqref{eq:model} in this section, but switch to a continuous $\pi_{\Theta}$ instead of the discrete ones considered in the previous parts. 

To be precise, we consider $\pi_{\Theta}$ that takes the following form: 
%
\begin{align}
\label{eq:pi-U-density}
	\pi_{\Theta}(\dd x) \propto e^{-U(x)} \dd x, 
\end{align}
%
where $U: \RR^n \to \RR$ has second order derivative that satisfies $|U''(x)| \leq C$ for all $x \in \RR^n$. We assume $\pi_{\Theta}$ has unit second moment and bounded fourth moment, but do not require it has bounded support. 

In this section, we consider non-symmetric $\pi_{\Theta}$. 
We comment that the symmetric $\pi_{\Theta}$ case can be conveniently handled via applying random sign flip to the sample generation process, as we have discussed in the previous sections.   

Next, we show that for a sufficiently large $\beta$, Condition \ref{cond:first-stationary-point} is always satisfied. 

\begin{lemma}
\label{lemma:large-beta-cond1}
	Assume $\pi_{\Theta}$ has finite fourth moment. Then, there exists $\beta_{\Theta}$ that depends only on $\pi_{\Theta}$, such that for all $\beta \geq \beta_{\Theta}$ we have Condition \ref{cond:first-stationary-point}. 
\end{lemma}
%
We defer the proof of \cref{lemma:large-beta-cond1} to Appendix \ref{sec:proof-lemma:large-beta-cond1}. \cref{lemma:large-beta-cond1} implies that Bayes AMP consistently estimates the posterior expectation vector $\E[\btheta \mid \bX, \by(t)]$ for all $\beta \geq \beta_{\Theta}$. 
We formally state this result below: 
%
\begin{lemma}
\label{lemma:general-spike-AMP-consistent}
	Assume the conditions of \cref{lemma:large-beta-cond1}. Recall that $\hat \bm_t^k$ is the $k$-th AMP iterate as defined in \cref{eq:general-AMP}. Then, for any $\eps > 0$, there exists $k_{\eps} \in \NN_+$, such that for all $k \geq k_{\eps}$, with probability $1 - o_n(1)$ we have 
	%
	\begin{align*}
		\frac{1}{n} \| \hat \bm_t^k - \bm_{\sB} \|_2^2 \leq \eps. 
	\end{align*} 
\end{lemma}
%
In this case, the following limit exists:  
%
\begin{align*}
	q_{\beta, t} = \lim_{n \to \infty} \E\left[ \|\E[\btheta \mid \bX, \by(t)]\|_2^2 \right] / n, 
\end{align*}
%
where $q_{\beta, t} = \E[\E[\Theta \mid \gamma_{\beta, t} \Theta + \sqrt{\gamma_{\beta, t}} G]^2]$ and $\gamma_{\beta, t} = \argmax_{\gamma > 0} \Phi(\gamma, \beta, t)$. Here, $(\Theta, G) \sim \pi_{\Theta} \otimes \normal(0, 1)$. 
In the sequel, we shall restrict the estimation procedure on the sphere that has the right radius $\SS_{\beta, t} = \{\bx \in \RR^n: \|\bx\|_2 = \sqrt{n q_{\beta, t}}\}$. 
Note that $q_{\beta, t}$ depends on $(\beta, t, \pi_{\Theta})$. Among them, $t$ is given, $\beta$ can be consistently estimated as a function of the top eigenvalue of $\bX$, and $\pi_{\Theta}$ can be consistently approximated via empirical Bayes approach.  

\subsubsection{TAP free energy on a sphere}


We then define the TAP free energy. For $\bm \in \RR^n$, let 
%
\begin{align*}
	\cF_{\TAP}(\bm; t, \bX, \by(t), \beta) = & - \frac{\beta}{2} \langle \bm, \bX \bm \rangle + \frac{\beta^2 (1 - q_{\beta, t})\|\bm\|_2^2}{2} + \sum_{i = 1}^n h(m_i, \beta^2 q_{\beta, t}) - \langle \by(t), \bm \rangle,  
\end{align*} 
%
where
%
\begin{align*}
	 h(m, w) = \sup_{\lambda} \left[ \lambda m - \phi(\lambda, w) \right], \qquad \phi(\lambda, w) = \log \int e^{\lambda \theta - w\theta^2 / 2} \pi_{\Theta}(\dd \theta). 
\end{align*}
%
Define $\bm_{\sB} = \E[\btheta \mid \bX, \by(t)]$ for the sake of simplicity. 
In the next lemma, we show that $\bm_{\sB}$ is an approximate stationary point of the TAP free energy. We prove the lemma in Appendix \ref{sec:proof-lemma:approximate-stationary}. 
%
\begin{lemma}
\label{lemma:approximate-stationary}
	Assume $\pi_{\Theta}$ satisfies \cref{eq:pi-U-density} and the conditions that follow, and $\beta \geq \beta_{\Theta}$. Then, $\bm_{\sB}$ is an approximate stationary point of the TAP free energy, in the sense that 
	%
	\begin{align*}
		\frac{1}{n} \|\nabla \cF_{\TAP} (\bm_{\sB}; t, \bX, \by(t), \beta)\|_2^2 = o_P(1). 
	\end{align*}
\end{lemma}
%
We then show that the TAP free energy is ``strongly convex'' in a neighborhood of $\bm_{\sB}$, if restricted to the sphere $\SS_{\beta, t}$. We delay the proof of the lemma to Appendix \ref{sec:proof-lemma:projected-hessian}. 
%
\begin{lemma}
\label{lemma:projected-hessian}
	We assume the conditions of \cref{lemma:approximate-stationary}. Then for a large enough $\beta$, there exists $r, \kappa > 0$, such that the following statement is true with probability $1 - o_n(1)$: 
	For all $\bm \in \mathsf{B}(\bm_{\sB}, \sqrt{n} r)$ and $\bx \perp \bm$, 
	%
	\begin{align*}
		\bx^{\top}\nabla^2 \cF_{\TAP} (\bm; t, \bX, \by(t), \beta) \bx \geq \kappa \|\bx\|_2^2. 
	\end{align*}
\end{lemma}

\subsubsection{Gradient descent on the  tangent space}

\cref{lemma:projected-hessian} motivates us to consider an algorithm that implements gradient descent on a tangent space. More precisely, for $\bm \in \SS_{\beta, t}$, we define $\bT_{\bm} \in \RR^{n \times (n - 1)}$, such that $\bT_{\bm}$ has orthonormal columns, and $\bm^{\top} \bT_{\bm} = \mathbf{0}$. Let $\cG_{\bm}: \RR^{n - 1} \mapsto \RR^n$, such that 
%
\begin{align*}
	\cG_{\bm}(\bw) =\sqrt{n q_{\beta, t}} \cdot \frac{\bm + \bT_{\bm} \bw}{\|\bm + \bT_{\bm} \bw \|_2}. 
\end{align*}
%
Next, we prove that for all $\bm$ that is sufficiently close to $\bm_{\sB}$, $\cG_{\bm}(\bw)$ is strongly convex in a small neighborhood of the origin. 
Formally speaking, we have the following lemma: 
%
\begin{lemma}
\label{lemma:tangent-space-convextiy}
	We assume the conditions of \cref{lemma:projected-hessian}. Recall that $\hat \bm_t^k$ is the $k$-th AMP iterate as defined in \cref{eq:general-AMP}. Then, there exists $k_{\ast} \in \NN_+$ that depends only on $(\beta, \pi_{\Theta})$, such that for all $k \geq k_{\ast}$, the following statement is true with probability $1 - o_n(1)$: There exists $R > 0$, such that the mapping $\bw \mapsto \cF_{\TAP}(\cG_{\hat \bm_t^k}(\bw); t, \bX, \by(t), \beta)$ is strongly convex on $\{\bw \in \RR^{n - 1}: \|\bw\|_2 \leq R\sqrt{n}\}$. Furthermore, if we denote the minimizer of this function on $\{\bw \in \RR^{n - 1}: \|\bw\|_2 \leq R \sqrt{n}\}$ by $\bw^{\ast}$, then $\|\bw^{\ast}\|_2 < R \sqrt{n}$, and 
	%
	\begin{align*}
		\frac{1}{\sqrt{n}}  \|\cG_{\hat \bm_t^k}(\bw^{\ast}) - \bm_{\sB}\|_2 = o_P(1). 
	\end{align*}
\end{lemma}
%
We prove \cref{lemma:tangent-space-convextiy} in Appendix \ref{sec:proof-lemma:tangent-space-convextiy}.  
\cref{lemma:tangent-space-convextiy} inspires us to design a two-stage algorithm to estimate the posterior expectation vector. In the first stage, we run Bayes AMP with a sufficient number of iterations. In the second stage, we run gradient descent on the tangent space associate with the Bayes AMP output. 

To be precise, we denote by $\hat \bm_t^k$ the output of certain Bayes AMP. We propose to implement gradient descent with $K_{\GD}$ steps and step size $\zeta$ on the tangent space associated with $\hat\bm_t^k$:
%
\begin{align}
\label{eq:GD-tangent-space}
\begin{split}
	& \bw^0 = \mathbf{0}_{n - 1}, \\
	& \bw^{i + 1} = \bw^i + \zeta \cdot \nabla_{\bw} \cF_{\TAP}(\cG_{\hat \bm_t^k}(\bw); t, \bX, \by(t), \beta) \big|_{\bw = \bw^i}, \qquad i = 0, 1, \cdots, K_{\GD} - 1.   
\end{split}
\end{align}
%
With \cref{lemma:tangent-space-convextiy}, we are ready to state our sampling algorithm.  
%
\begin{algorithm}
\caption{Diffusion-based sampling for spiked models with a continuous prior}\label{alg:general-sampling-continuous}
\textbf{Input: }Data $\bX$, parameters $(\beta, K_{\AMP}, K_{\GD}, \zeta, L, \delta)$;	
\begin{algorithmic}[1]
	\For{$\ell = 0,1,\cdots, L - 1$}
		\State Draw $\bw_{\ell + 1} \sim \normal(0, \id_n)$ independent of everything so far;
		\State Let $\hat \bm_{\ell \delta}^{K_{\AMP}}(\hat \by_{\ell})$ be the output of the Bayes AMP algorithm \eqref{eq:general-AMP} with $K_{\AMP}$ iterations;
		\State Let $\hat\bm(\hat \by_{\ell},\ell\delta)$ be the output of algorithm \eqref{eq:GD-tangent-space} with AMP output $\hat \bm_{\ell \delta}^{K_{\AMP}}(\hat \by_{\ell})$, number of gradient descent steps $K_{\GD}$ and step size $\zeta$;
		\State Update $\hat \by_{\ell + 1} = \hat \by_{\ell} + \hat\bm(\hat \by_{\ell},\ell\delta) \delta + \sqrt{\delta} \bw_{\ell + 1}$;	
	\EndFor
\State \Return $\btheta^{\salg}  = \hat\bm(\hat \by_{L},L\delta)$; 
\end{algorithmic}
\end{algorithm}  

We state below theoretical guarantee for \cref{alg:general-sampling-continuous}. We prove the theorem in Appendix \ref{thm:spiked-continious}. 


\begin{theorem}
\label{thm:spiked-continuous}
	We denote by $\mu_{\bX}^{\salg}$ the law of $\btheta^{\salg}$ from \cref{alg:general-sampling-continuous}, and denote by $\mu_{\bX}$ the posterior distribution of $\btheta$ upon observing $\bX$. We assume that $\pi_{\Theta}(\dd x) \propto e^{-U(x)} \dd x$ with $\|U''\|_{\infty} \leq C$ for some positive constant $C$.
	Then, there exists $\beta_{\Theta} > 0$ that is a function of $\pi_{\Theta}$, such that for all $\beta \geq \beta_{\Theta}$ the following statements are true: For any $\xi > 0$, there exist $(K_{\AMP}, K_{\GD}, \zeta, L, \delta)$ that depends only on $(\beta, \pi_{\Theta})$, such that with probability $1 - o_n(1)$ over the randomness of $\bX$, we have
	%
	\begin{align*}
			W_{2, n} (\mu_{\bX}, \mu_{\bX}^{\mathsf{alg}}) \leq \xi. 
		\end{align*}  
\end{theorem} 



